A Unified Analysis of Four Cosmic Shear Surveys

In the past few years, several independent collaborations have presented cosmological constraints from tomographic cosmic shear analyses. These analyses differ in many aspects: the datasets, the shear and photometric redshift estimation algorithms, the theory model assumptions, and the inference pipelines. To assess the robustness of the existing cosmic shear results, we present in this paper a unified analysis of four of the recent cosmic shear surveys: the Deep Lens Survey (DLS), the Canada-France-Hawaii Telescope Lensing Survey (CFHTLenS), the Science Verification data from the Dark Energy Survey (DES-SV), and the 450 deg$^{2}$ release of the Kilo-Degree Survey (KiDS-450). By using a unified pipeline, we show how the cosmological constraints are sensitive to the various details of the pipeline. We identify several analysis choices that can shift the cosmological constraints by a significant fraction of the uncertainties. For our fiducial analysis choice, considering a Gaussian covariance, conservative scale cuts, assuming no baryonic feedback contamination, identical cosmological parameter priors and intrinsic alignment treatments, we find the constraints (mean, 16% and 84% confidence intervals) on the parameter $S_{8}\equiv \sigma_{8}(\Omega_{\rm m}/0.3)^{0.5}$ to be $S_{8}=0.94_{-0.045}^{+0.046}$ (DLS), $0.66_{-0.071}^{+0.070}$ (CFHTLenS), $0.84_{-0.061}^{+0.062}$ (DES-SV) and $0.76_{-0.049}^{+0.048}$ (KiDS-450). From the goodness-of-fit and the Bayesian evidence ratio, we determine that amongst the four surveys, the two more recent surveys, DES-SV and KiDS-450, have acceptable goodness-of-fit and are consistent with each other. The combined constraints are $S_{8}=0.79^{+0.042}_{-0.041}$, which is in good agreement with the first year of DES cosmic shear results and recent CMB constraints from the Planck satellite.

==> Makefile <==
# To make the document with the default settings:
# > make
#
# To make with a specific format:
# > make <format>
#
# To tar up a flat version of a specific format:
# > make <format> tar
#
# Alex Drlica-Wagner: https://github.com/DarkEnergyScienceCollaboration/start_paper/issues/new?body=@kadrlica

# Primary file names - avoid cookiecutter variables, to enable `make
# upgrade` to cleanly over-write this Makefile...
main=main
outname=$(notdir $(shell pwd))

# LATEX environment variables
export TEXINPUTS:=./texmf/styles/:./tables/:
export BSTINPUTS:=./texmf/bib/:

# LaTeX journal class switcher flags
# apj=\def\flag{apj}
# apjl=\def
# mnras=\def\flag{mnras}

# Submission flags (these need some thought)
# arxiv=\def\flag{emulateapj}
# submit=${aastex}
# draft=\def\linenums{\linenumbers}

# Files to copy when making tarball
tardir=tmp
figdir=./figures
figures=$(figdir)/*.{png,jpg,pdf}
tabdir=./tables
tables=$(tabdir)/*.tex
styles=./texmf/styles/*.{sty,cls}
bibs=./texmf/bib/*.bst
source=$(main).{tex,bbl,bib} lsstdesc.bib macros.tex authors.tex acknowledgments.tex

tarfiles=$(figures) $(tables) $(styles) $(bibs) $(source)

# Interpret `make` with no target as `make tex`, a latex Note
all: export flag = \def\flag{tex}
all: main copy

copy:
	cp ${main}.pdf ${outname}.pdf

touch:
	touch ${main}.tex

#http://journals.aas.org/authors/aastex/linux.html
#change the compiler call to allow a "." file
# {% raw %}
main :
	latexmk -g -pdf  \
	-pdflatex='openout_any=a pdflatex %O -interaction=nonstopmode "${flag}\input{%S}"'  \
	${main}
# {% endraw %}

tar : main
	mkdir -p ${tardir}
	cp ${tarfiles} ${tardir} | true
	cp ${outname}.pdf ${tardir}/${outname}.pdf
	cd ${tardir} && tar -czf ../${outname}.tar.gz . && cd ..
	rm -rf ${tardir}

# http://stackoverflow.com/q/8028314/
TARGETS=apj apjl prd prl mnras tex
$(TARGETS): export flag = \def\flag{$(@)}
$(TARGETS):
	$(MAKE) -e main
	$(MAKE) -e copy
	$(MAKE) -e tar
# NB. the 'tex' target doesn't actually do anything in docswitch - make
# with no target compiles PDF out of main.tex using lsstdescnote.cls
# (which is to say, by default we assume you are writing an LSST
# DESC Note in latex format).

tidy:
	rm -f *.log *.aux *.out *.dvi *.synctex.gz *.fdb_latexmk *.fls
	rm -f *.bbl *.blg *Notes.bib ${main}.pdf

clean: tidy
	rm -f ${outname}.pdf ${outname}.tar.gz

# Update the tex styles etc:

baseurl=https://raw.githubusercontent.com/DarkEnergyScienceCollaboration/start_paper/master/%7B%7Bcookiecutter.folder_name%7D%7D

UPDATES=\
texmf/bib/apj.bst \
texmf/bib/mnras.bst \
texmf/styles/aas_macros.sty \
texmf/styles/aastex.cls \
texmf/styles/aastex61.cls \
texmf/styles/aps_macros.sty \
texmf/styles/docswitch.sty \
texmf/styles/emulateapj.cls \
texmf/styles/mnras.cls \
texmf/styles/lsstdescnote.cls \
.logos/desc-logo-small.png \
.logos/desc-logo.png \
.logos/header.png \
lsstdesc.bib \
.travis.yml \
figures/example.png

.PHONY: $(UPDATES)
$(UPDATES):
	curl -s -S -o $(@) ${baseurl}/$(@)
	@echo " "

update:
	@echo "\nOver-writing LaTeX style files with the latest versions: \n"
	@mkdir -p .logos figures texmf/styles texmf/bib
	$(MAKE) $(UPDATES)

# Get fresh copies of the templates etc, for reference:

TEMPLATES=\
acknowledgments.tex \
authors.tex \
macros.tex \
main.ipynb \
main.md \
main.rst \
main.tex \
main.bib

.PHONY: $(TEMPLATES) templates
$(TEMPLATES):
	curl -s -S -o templates/$(@) ${baseurl}/$(@)
	@echo " "

templates:
	@echo "\nDownloading the latest versions of the template files, for reference: \n"
	@mkdir -p templates
	$(MAKE) $(TEMPLATES)
	$(MAKE) new
	ls templates/*

# Get a template copy of the latest Makefile, for reference:
.PHONY: new
new:
	@echo "\nDownloading the latest version of the Makefile, for reference: \n"
	@mkdir -p templates
	curl -s -S -o templates/Makefile ${baseurl}/Makefile
	@echo " "

# Over-write this Makefile with the latest version:
.PHONY: upgrade
upgrade:
	@echo "\nDownloading the latest version of the Makefile: \n"
	curl -s -S -o Makefile ${baseurl}/Makefile
	@echo "\nNow get the latest styles and templates with\n\n    make update\n    make templates\n"


==> authors.tex <==
\author{Chihway Chang}
\affiliation{Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637}
\author{Michael Wang}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{Scott Dodelson}
% below is alphabetical order for now
%\author{Sebastian Bouquet}
\author{Tim Eifler}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\affiliation{Department of Physics, California Institute of Technology, Pasadena, CA 91125, USA}
\author{Catherine Heymans}
\affiliation{Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK}
\author{Michael Jarvis}
\affiliation{Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\author{M. James Jee}
\affiliation{Department of Astronomy, Yonsei University, Yonsei-ro 50, Seoul, Korea}
\affiliation{Department of Physics, University of California, Davis, California, USA}
\author{Shahab Joudaki}
\affiliation{Department of Physics, University of Oxford, Denys Wilkinson Building, Keble Road, Oxford OX1 3RH, UK}
\author{Elisabeth Krause}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\affiliation{Department of Physics, California Institute of Technology, Pasadena, CA 91125, USA}
%\author{Francois Lanusse}
%\affiliation{McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA}
\author{Alex Malz}
\affiliation{Center for Cosmology and Particle Physics, New York University, 726 Broadway, New York, 10003, USA}
\affiliation{Department of Physics, New York University, 726 Broadway, New York, 10003, USA}
\author{Rachel Mandelbaum}
\affiliation{McWilliams Center for Cosmology, Department of Physics, Carnegie Mellon University, Pittsburgh, PA 15213, USA}
%\author{Javier Sanchez}
\author{Irshad Mohammed}
\affiliation{Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL 60510, USA}
\author{Michael Schneider}
\affiliation{Lawrence Livermore National Laboratory, Livermore, CA 94551, USA}
\author{Melanie Simet}
\affiliation{Jet Propulsion Laboratory, California Institute of Technology, 4800 Oak Grove Dr., Pasadena, CA 91109, USA}
\affiliation{University of California, Riverside, 900 University Avenue, Riverside, CA 92521, USA}
\author{Michael Troxel}
\affiliation{Center for Cosmology and Astro-Particle Physics, The Ohio State University, Columbus, OH 43210, USA}
\affiliation{Department of Physics, The Ohio State University, Columbus, OH 43210, USA}
\author{Joe Zuntz}
\affiliation{Institute for Astronomy, University of Edinburgh, Edinburgh EH9 3HJ, UK}

